Following the Human Thread in Social Navigation

The success of collaboration between humans and robots in shared environments relies on the robot's real-time adaptation to human motion. Specifically, in Social Navigation, the agent should be close enough to assist but ready to back up to let the human move freely, avoiding collisions. Human trajectories emerge as crucial cues in Social Navigation, but they are partially observable from the robot's egocentric view and computationally complex to process. We present the first Social Dynamics Adaptation model (SDA) based on the robot's state-action history to infer the social dynamics. We propose a two-stage Reinforcement Learning framework: the first learns to encode the human trajectories into social dynamics and learns a motion policy conditioned on this encoded information, the current status, and the previous action. Here, the trajectories are fully visible, i.e., assumed as privileged information. In the second stage, the trained policy operates without direct access to trajectories. Instead, the model infers the social dynamics solely from the history of previous actions and statuses in real-time. Tested on the novel Habitat 3.0 platform, SDA sets a novel state-of-the-art (SotA) performance in finding and following humans. The code can be found at https://github.com/L-Scofano/SDA.

==> tables/ablation_deployment.tex <==
\begin{table}[]
\centering
\setlength{\tabcolsep}{3.5pt} % Adjust the space between columns here
\caption{Main results for Social Navigation \LS{change caption, add citation in tab., eventually add stage 1 in another table or highlight it in grey}. We might want to add the SD in the table. The * means that the variable is latent and distilled. rr = refresh rate}
\begin{tabular}{c|cccccccc}
\hline
  rr & S $\uparrow$ & SPS $\uparrow$ & F $\uparrow$ & CR $\downarrow$ & BYR & TD $\downarrow$ & FD $\downarrow$ & NSS $\uparrow$ \\ \hline
 1 & \textbf{0.88} & 0.44 &  0.39   & \textbf{0.62}  &  0.09  &  4.23   &  1.76  &  0.42   \\
 1/2 & 0.87 & 0.45  &  \textbf{0.44}   & 0.63  &  0.17  &  3.80   &  1.49  &  0.48   \\
 1/100 & 0.85 & 0.45  &  0.43   & 0.64  &  0.16  &  3.86   &  1.51  &  0.46   \\
1/1000 & ? & ? & ? & ? & ? & ? & ? & ?  \\

\hline
\end{tabular}
\label{tab:ablation_deploy}
\end{table}

==> tables/main_table.tex <==
\begin{table}[]
\centering
\setlength{\tabcolsep}{3.5pt} % Adjust the space between columns here
\caption{Main results for Social Navigation. Within the table, GT denotes ground truth data, L represents latent information, and A the adapted information.}
%\FG{add a footnote to "Baseline+proximity~\cite{cancelli23}" to indicate "Code refactored and adapted from \cite{cancelli23} to Habitat 3.0". In the case of baseline+proximity, we might not need to again cite habitat. Removing the citation of habitat makes it look like another entry/another method in the table}
\begin{tabular}{l|cc|ccccc}
\hline
Models  & hGPS & traj. & S $\uparrow$ & SPS $\uparrow$ & F $\uparrow$ & CR $\downarrow$ & ES $\uparrow$ \\ \hline
Heuristic Expert~\cite{puig2023habitat}  & - & - & 1.00  &  0.97   & 0.51  &  0.52 &  - \\ \hline \hline
Baseline~\cite{puig2023habitat}    & GT & & 0.97  &   0.65  & 0.44  &  0.51  &   0.55*  \\
Baseline+Proximity~\cite{cancelli23} flag True\footnote{Code refactored and adapted from \cite{cancelli23} to Habitat 3.0 flag True}  & GT & & 0.96  &   0.70  & 0.54  &  0.32  &   0.63  \\
Baseline+Proximity~\cite{cancelli23} Cineca \footnote{Code refactored and adapted from \cite{cancelli23} to Habitat 3.0}  & GT & & 0.97  &   ?  & 0.57  &  0.58  &   0.63  \\
\modelname - S1  &  GT  & L &  0.96 &  0.64   & 0.46  &  0.65 &  0.49   \\ 
%\modelname - S1 & & L & 0.88 & 0.44  &  0.44   &  0.59 &   0.50   \\
\modelname - S1 Cineca & & L & 0.92 & 0.46  &  0.44   &  0.61 &   0.50   \\
\modelname - S1  & L & & 0.93  &  0.62  & 0.46  &  0.64  &  0.48  \\
\modelname - S1   & L & L & 0.94  &  0.58  & 0.45  &  0.64  &   0.52  \\ \hline \hline
Baseline~\cite{puig2023habitat}  & & & 0.76  &  0.34   & 0.29  &  \textbf{0.48}  & 0.42*  \\
Baseline+Proximity~\cite{cancelli23} flag True & & & 0.86  &  0.45   & 0.41  &  0.38  & 0.45  \\
Baseline+Proximity~\cite{cancelli23} Cineca & & & 0.85  &  ?  & 0.41  &  0.58  & 0.45  \\
% \cite{puig2023habitat} reprod.  & & & 0.76  &  0.37   & 0.29  &  0.53  &  0.14   & 5.18   &  1.64  & 0.42    \\
%\modelname - S2 Visnu & & A & \textbf{0.88} & \textbf{0.44}  &  \textbf{0.39}   & 0.62  &  0.42   \\ 
\modelname - S2 Cineca  & & A & \textbf{0.91} & \textbf{0.45}  &  \textbf{0.39}   & 0.57  &  0.43   \\ 
\modelname - S2 Cineca flag True & & A & \textbf{0.90} & \textbf{?}  &  \textbf{0.36}   & 0.41  &  0.45   \\ 
\hline
\modelname - S2 & A &  & 0.7 &  0.31  & 0.05  &  0.7 & 0 \\
\modelname - S2 & A & A & 0.57 & 0.21  &  0.05   & 0.3  &  0.002   \\
\hline
\end{tabular}
\label{tab:main}
\end{table}

==> tables/main_table_extra.tex <==
\begin{table}[]
\centering
\setlength{\tabcolsep}{3.5pt} % Adjust the space between columns here
\caption{Results for Social Navigation using Humanoid GPS both for us and for them \LS{change caption, add citation in tab., eventually add stage 1 in another table or highlight it in grey. This might be added in the main table}}
\begin{tabular}{l|cccccccc}
\hline
Models  & S $\uparrow$ & SPS $\uparrow$ & F $\uparrow$ & CR $\downarrow$ & BYR & TD $\downarrow$ & FD $\downarrow$ & NSS $\uparrow$ \\ \hline
Heuristic Expert     & 1.00  &  0.97   & 0.51  &  0.52  &  0.24   & 2.56   &  1.72  &  na   \\
Habitat 3.0 E2E      &   &     &   &    &     &    &    &     \\
Ours                 &   &     &   &    &     &    &    &     \\
Ours Stage 1         &   &     &   &    &     &    &    &     \\
\hline
\end{tabular}
\label{tab:egopose}
\end{table}




==> tables/rebuttal/ablation_different_t.tex <==
\begin{table}[!ht]
\centering
\setlength{\tabcolsep}{3.5pt} % Adjust the space between columns here
\caption{Trajectory leght ablation study \\ extending Table 3 of the main paper. %\LS{Since we have this table in the main paper (Tab.3), should we just compare t=1 and t=20 (Proposed) and discard the rest?}\IS{keep them all and say that it extends Table 3 from main paper}
}
\begin{tabular}{l|ccccc}
\hline
\# states considered  & S $\uparrow$ & SPS $\uparrow$ & F $\uparrow$ & CR $\downarrow$ & ES $\uparrow$ \\ \hline
1                 &  0.55$^{\pm0.01}$   &   0.14$^{\pm0.02}$  & 0.03$^{\pm0.01}$   &  0.75$^{\pm0.01}$  & 0.03$^{\pm0.01}$     \\
%5                 &  0.62$^{\pm0.01}$   &   0.25$^{\pm0.02}$  & 0.05$^{\pm0.01}$   &  0.64$^{\pm0.01}$  & 0.06$^{\pm0.01}$     \\
20 (\textit{Proposed})         &  \textbf{0.91}$^{\pm0.01}$ & \textbf{0.45}$^{\pm0.01}$  &  \textbf{0.39}$^{\pm0.01}$   & \textbf{0.57}$^{\pm0.02}$  &  \textbf{0.43}$^{\pm0.02}$  \\
%50                &  0.70$^{\pm0.02}$   &   0.29$^{\pm0.02}$  &  0.08$^{\pm0.02}$  &  0.78$^{\pm0.02}$  &  0.08$^{\pm0.01}$ \\
\hline
\end{tabular}
\label{tab:ablation_t}
\end{table}

==> tables/rebuttal/aligned_t_encoder.tex <==
\noindent\begin{minipage}[!t]{.5\textwidth}%
\centering
\captionof{table}{Trajectory leght ablation study \\ extending Table 3 of the main paper.}
% \FG{This table is very small, it might be too small. But do we need to keep the neurips paper margins in this pdf? If not, I'd enlarge the editable area in the page and re-enlarge these tables.}%
\label{tab:ablation_t}
\resizebox{0.92\textwidth}{!}{
\begin{tabular}{l|ccccc}
\hline
\# states considered  & S $\uparrow$ & SPS $\uparrow$ & F $\uparrow$ & CR $\downarrow$ & ES $\uparrow$ \\ \hline
1                 &  0.55$^{\pm0.01}$   &   0.14$^{\pm0.02}$  & 0.03$^{\pm0.01}$   &  0.75$^{\pm0.01}$  & 0.03$^{\pm0.01}$     \\
%5                 &  0.62$^{\pm0.01}$   &   0.25$^{\pm0.02}$  & 0.05$^{\pm0.01}$   &  0.64$^{\pm0.01}$  & 0.06$^{\pm0.01}$     \\
20 (\textit{Proposed})         &  \textbf{0.91}$^{\pm0.01}$ & \textbf{0.45}$^{\pm0.01}$  &  \textbf{0.39}$^{\pm0.01}$   & \textbf{0.57}$^{\pm0.02}$  &  \textbf{0.43}$^{\pm0.02}$  \\
%50                &  0.70$^{\pm0.02}$   &   0.29$^{\pm0.02}$  &  0.08$^{\pm0.02}$  &  0.78$^{\pm0.02}$  &  0.08$^{\pm0.01}$ \\
\hline
\end{tabular}}%
%\hfill%
\end{minipage}%
\begin{minipage}[!t]{.5\textwidth}%
\captionof{table}{Ablation on the type of\\ encoder to consider during Stage 1.}%
%\hfill%
\label{tab:ablation_enc}
\resizebox{0.92\textwidth}{!}{
\begin{tabular}{l|ccccc}
\hline
Encoder Type & S $\uparrow$ & SPS $\uparrow$ & F $\uparrow$ & CR $\downarrow$ & ES $\uparrow$ \\ \hline

MLP (\textit{Proposed})         &  \textbf{0.91}$^{\pm0.01}$ & \textbf{0.45}$^{\pm0.01}$  &  \textbf{0.39}$^{\pm0.01}$   & \textbf{0.57}$^{\pm0.02}$  &  \textbf{0.43}$^{\pm0.02}$   \\
Transformer                &  0.85$^{\pm0.01}$   &   0.15$^{\pm0.02}$  & 0.27$^{\pm0.01}$   &  0.76$^{\pm0.01}$  & 0.12$^{\pm0.01}$     \\
\hline
\end{tabular}}
%\vspace{-.3cm}
\end{minipage}%



==> tables/rebuttal_iclr/random_speed.tex <==
\begin{table}[!ht]
\centering
\setlength{\tabcolsep}{3.5pt} % Adjust the space between columns here
\caption{Comparison of SDA Stage 2 performances using constant human speed (h.speed) or random human speed in the simulator.}
\begin{tabular}{l|c|ccccc}
\hline
Model  & h.speed & S $\uparrow$ & SPS $\uparrow$ & F $\uparrow$ & CR $\downarrow$ & ES $\uparrow$ \\ \hline

\modelname - S2  & constant & \textbf{0.91}$^{\pm0.01}$ & \textbf{0.45}$^{\pm0.01}$  &  \textbf{0.39}$^{\pm0.01}$   & 0.57$^{\pm0.02}$  &  0.43$^{\pm0.02}$   \\ 
\modelname - S2 & constant/2 & 0.87$^{\pm0.01}$   &   0.57$^{\pm0.02}$  & 0.28$^{\pm0.01}$   &  \textbf{0.13}$^{\pm0.01}$  & \textbf{0.70}$^{\pm0.01}$   \\
\modelname - S2 & random & 0.90$^{\pm0.01}$   &   \textbf{0.45}$^{\pm0.02}$  & 0.25$^{\pm0.01}$   &  0.48$^{\pm0.01}$  & 0.40$^{\pm0.01}$   \\

\hline
\end{tabular}
\label{tab:rebuttal_speed}
\end{table}

==> tables/rebuttal_iclr/rebuttal_multi_human.tex <==
\begin{table}[!h]
\centering
\setlength{\tabcolsep}{3.5pt} % Adjust the space between columns here
\caption{Comparison of SDA performances on Habitat 3.0 with a single and with multiple people.}
\begin{tabular}{l|ccccc}
\hline
 & S $\uparrow$ & SPS $\uparrow$ & F $\uparrow$ & CR $\downarrow$ & ES $\uparrow$ \\ \hline

\textit{SDA - S2 single-human} &  \textbf{0.91}$^{\pm0.01}$ & \textbf{0.45}$^{\pm0.01}$  &  \textbf{0.39}$^{\pm0.01}$   & 0.57$^{\pm0.02}$  &  \textbf{0.43}$^{\pm0.02}$   \\
Baseline single-human & 0.76$^{\pm0.02}$  &  0.34$^{\pm0.01}$   & 0.29$^{\pm0.01}$  &  \textbf{0.48}$^{\pm0.03}$  & 0.40$^{\pm0.02}$  \\
\textit{SDA - S2  two-humans} &  0.80$^{\pm0.01}$   &   0.41$^{\pm0.02}$  & 0.18$^{\pm0.01}$   &  0.68$^{\pm0.01}$  & 0.20$^{\pm0.01}$   \\
Baseline two-humans &  0.76$^{\pm0.01}$   &   0.36$^{\pm0.02}$  & 0.09$^{\pm0.01}$   &  0.80$^{\pm0.01}$  & 0.11$^{\pm0.01}$   \\
\textit{SDA - S2 three-human}s &  0.70$^{\pm0.01}$   &   0.38$^{\pm0.02}$  & 0.12$^{\pm0.01}$   &  0.78$^{\pm0.01}$  & 0.15$^{\pm0.01}$   \\
Baseline three-humans &  0.67$^{\pm0.01}$   &   0.36$^{\pm0.02}$  & 0.07$^{\pm0.01}$   &  0.83$^{\pm0.01}$  & 0.09$^{\pm0.01}$   \\
\hline
\end{tabular}
\label{tab:multi}
\end{table}


==> tables/rebuttal_iclr/rebuttal_test.tex <==
\begin{table}[h!]
\centering
\begin{tabular}{@{}cccccc@{}}
\toprule
\textbf{Metric} & \textbf{Baseline + Proximity} & \textbf{SDA - S2} & \textbf{t-statistic} & \textbf{p-value} & \textbf{Significance} \\ \midrule
S               & $0.85 \pm 0.02$               & $0.91 \pm 0.01$   & $-8.49$              & $1.03 \times 10^{-6}$ & Significant          \\
SPS               & $0.41 \pm 0.02$               & $0.45 \pm 0.01$   & $-5.66$              & $7.32 \times 10^{-5}$ & Significant          \\
F               & $0.37 \pm 0.01$               & $0.39 \pm 0.01$   & $-4.47$              & $2.95 \times 10^{-4}$ & Significant          \\
CR               & $0.58 \pm 0.02$               & $0.54 \pm 0.02$   & $4.47$               & $2.95 \times 10^{-4}$ & Significant          \\
ES               & $0.42 \pm 0.01$               & $0.45 \pm 0.02$   & $-4.24$              & $9.24 \times 10^{-4}$ & Significant          \\ \bottomrule
\end{tabular}
\caption{Updated t-statistics and p-values for the comparison of methods.}
\label{tab:updated_results}
\end{table}
